SweLL on the rise: Swedish Learner Language corpus for European Reference Level studies

We present a new resource for Swedish, SweLL, a corpus of Swedish Learner essays linked to learners' performance according to the Common European Framework of Reference (CEFR). SweLL consists of three subcorpora - SpIn, SW1203 and Tisus, collected from three different educational establishments. The common metadata for all subcorpora includes age, gender, native languages, time of residence in Sweden, type of written task. Depending on the subcorpus, learner texts may contain additional information, such as text genres, topics, grades. Five of the six CEFR levels are represented in the corpus: A1, A2, B1, B2 and C1 comprising in total 339 essays. C2 level is not included since courses at C2 level are not offered. The work flow consists of collection of essays and permits, essay digitization and registration, meta-data annotation, automatic linguistic annotation. Inter-rater agreement is presented on the basis of SW1203 subcorpus. The work on SweLL is still ongoing with more than 100 essays waiting in the pipeline. This article both describes the resource and the "how-to" behind the compilation of SweLL.

==> Makefile <==
FILE ?= elex2015
BIBTEX := $(wildcard $(FILE).bib) 

all: dvi pdf ps
clean:
	@echo -e "\n*****Deleting *.aux $$FILE.pdf *.dvi *.ps *.log *.idx *.ind *.toc *.out *.ilg *.blg *.bbl *.tfm *pk tmp.mf\n"
	-rm *.aux $$FILE.pdf *.dvi *.ps *.log *.idx *.ind *.toc *.out *.ilg *.blg *.bbl *.tfm *pk tmp.mf *.nav *.snm
	@echo -e "\n*****Finished deleting!\n"
viewpdf: pdf
	@okular $(FILE).pdf &
viewps: ps
	@kghostview $(FILE).ps & 
viewdvi: dvi
	@kdvi $(FILE).dvi &
dvi: $(FILE).dvi
pdf: $(FILE).pdf
ps: $(FILE).ps
pdfopt: pdf
	@echo -e "\n******Optimizing PDF\n"
	mv $(FILE).pdf $(FILE)-in.pdf
	pdfopt $(FILE)-in.pdf $(FILE).pdf
	rm $(FILE)-in.pdf
	@echo -e "\n******Finished optimizing!\n"
$(FILE).pdf: vlna bibtex $(FILE).tex
	@echo -e "\n******Creating PDF\n"
	pdflatex $(FILE).tex
#	@while grep -qs 'LaTeX Warning:.*references' $(FILE).log; do echo; pdflatex -output-format=pdf $(FILE).tex; done
	@echo -e "\n******Finished creating PDF!\n"
$(FILE).dvi: vlna bibtex $(FILE).tex
	@echo -e "\n******Creating DVI\n"
	pdflatex -output-format=dvi $(FILE).tex
	@while grep -qs 'LaTeX Warning:.*references' $(FILE).log; do echo; latex $(FILE).tex; done
	@echo -e "\n******Finished creating DVI!\n"
$(FILE).ps: bibtex $(FILE).dvi
	@echo -e "\n******Creating PS\n"
	dvips $(FILE).dvi -o
	@echo -e "\n******Finished creating PS\n"
ifeq ($(strip $(BIBTEX)),) 
bibtex:
	@echo -e "\n******No bibtex found\n"
else
bibtex: $(FILE).bib
	@echo -e "\n******Making bibtex\n"
	pdflatex -output-format=pdf $(FILE).tex
	bibtex $(FILE)
endif
vlna:
	vlna -m -n -v KkSsZzVvOoIiAaUu $(FILE).tex

